Reversing Place Transition Nets

Petri nets are a well-known model of concurrency and provide an ideal setting for the study of fundamental aspects in concurrent systems. Despite their simplicity, they still lack a satisfactory causally reversible semantics. We develop such semantics for Place/Transitions Petri nets (P/T nets) based on two observations. Firstly, a net that explicitly expresses causality and conflict among events, for example an occurrence net, can be straightforwardly reversed by adding a reverse transition for each of its forward transitions. Secondly, given a P/T net the standard unfolding construction associates with it an occurrence net that preserves all of its computation. Consequently, the reversible semantics of a P/T net can be obtained as the reversible semantics of its unfolding. We show that such reversible behaviour can be expressed as a finite net whose tokens are coloured by causal histories. Colours in our encoding resemble the causal memories that are typical in reversible process calculi.

==> cau_proof.tex <==
% !TEX root = main.tex

\section{Proofs}\label{app:proof}
We start with the proof of a simple version of Square Lemma from Section 2. 
Note that $\tr t$ and $\tr t'$ are forward transitions.
\begin{lm}{\ref{lem:SL-F}}
Let $\tr t$ and $\tr t'$ be coinitial concurrent transitions. Then, there exist transitions
$\tr t_1$ and $\tr t_1'$ such that $\tr t;\tr t_1'$ and $\tr t';\tr t_1$ are cofinal.
\end{lm}
\begin{proof}
Since $\tr t$ and $\tr t'$ be coinitial they do not cause each other. To be concurrent they also
cannot be in an immediate conflict, implying that we can write them as
$(N, m\oplus m'\oplus m'')\red (N, m_1\oplus m'\oplus m'')$ and
$(N, m\oplus m'\oplus m'')\red[\tr t'] (N, m\oplus m_1'\oplus m'')$, where
$m$ and $m'$ do not overlap. Clearly then these are valid transitions:
$(N, m\oplus m_1'\oplus m'')\red[\tr t_1] (N, m_1\oplus m_1'\oplus m'')$ and
$(N, m_1\oplus m'\oplus m'')\red[\tr t_1'] (N, m_1\oplus m_1'\oplus m'')$. Since $\tr t_1$ and $\tr t_1'$
are cofinal (resulting in $(N, m_1\oplus m_1'\oplus m'')$), we obtain $\tr t;\tr t_1'$
and $\tr t';\tr t_1$ are cofinal.
\end{proof}

We now report the proofs of the main Lemmas/Theorems of Section~\ref{sec:prop}.

First, we have a lemma which is instrumental for the
proof of causal-consistent reversibility in reversible calculi~\cite{rccs,rhotcs}. Here,
each of $t$ and $t'$ is either a forward or reverse transition.
\begin{lm}{\ref{lem:SL-all}}
Let\; $t$ and $t'$ be coinitial concurrent transitions. Then, there exist transitions
$t_1$ and $t_1'$ such that $t;t_1'$ and $t';t_1$ are cofinal.
\end{lm}
%
\begin{proof}
We consider three cases when $t$ and $t'$ are
coinitial concurrent transitions. If $t$ and $t'$ are both forward then we are done by
lemma~\ref{lem:SL-F}. If $t$ and $t'$ are both reverse, then since they are cointial 
they cannot cause one another.
They cannot be in an immediate conflict because this would imply a backward conflict on 
their forward versions (which we do not have in occurrence nets). So, $t, t'$ do not share 
tokens in their preplaces. Hence, we can write $t, t'$ correspondingly as we wrote
$\tr t, \tr t'$ in the proof of lemma~\ref{lem:SL-F}. The rest of the case follows
correspondingly as in the proof of lemma~\ref{lem:SL-F}. 
If $t$ is a transition and $t'$ is a reverse transition,
then since they are coinitial they cannot cause one another. Hence, for $t$ and $t'$ to be concurrent we require
$\rev{t'}\not\preceq t$. This means that the preplaces of $t$ do not overlap with the postplaces of $\rev{t'}$,
hence the preplaces of $t$ do not overlap with the preplaces of $t'$. We then finish as in the proof of
lemma~\ref{lem:SL-F}.
\end{proof}


\begin{lm}{\ref{lm:rearranging}}
Let $\trace$ be a trace. There exist two forward traces $\trace_1$ and $\trace_2$
such that $\trace \ceq \rev{\trace_1};\trace_2$.
\end{lm}
\begin{proof}
The proof is by lexicographic induction on the length of $\trace$ and on the distance between 
the beginning of $\trace$ and the \emph{earliest pair} of firings in $\trace$ of the form 
$\tr{t_1};\rev{\tr{t_2}}$, where $\tr{t_1}$ and $\tr{t_2}$ are forward. If such pair does not exist, 
then the result follows immediately. If there exists one such pair we have two possibilities: 
either the two firings are concurrent or they are not.

%$\tr{t_1}\preceq \tr{t_2}$.
%$\postS{\tr{t_1}}\cap \preS{\rev{\tr{t_2}}} \neq \emptyset$.  
In the first case, this implies that
 $\preS{\tr{t_1}}\cap \preS{\rev{\tr{t_2}}} = \emptyset$. By exploiting the property of \m
traces we can swap the two firings, 
obtaining a later earliest pair contradicting our assumption. 
The result then follows by induction since swapping firings keeps the total length 
of the trace unchanged. 

If the two firings are not concurrent we have four cases:
\begin{enumerate}

\item $\tr{t_1}\prec \rev{\tr{t_2}} $, this implies
that $\postS{\tr{t_1}} \cap \preS{\rev{\tr{t_2}}} \neq \emptyset$ and that 
$\postS{\tr{t_1}}\cap \postS{\tr{t_2}} \neq \emptyset$. 
This means that there is a backward conflict between $\tr{t_1}$ and
$\tr{t_2}$. By definition occurrence nets are backward conflict free: contradiction.
%


\Comment{\item $\rev{\tr{t_2}} \prec{ \tr{t_1}} $, 
this implies
that $\postS{\rev{\tr{t_2}}}\cap \preS{\tr{t_1}} \neq \emptyset$,
and that $\preS{\tr{t_2}}\cap \preS{\tr{t_1}}\neq \emptyset$. For simplicity
we will consider transitions that consume one token, but the general case is similar.
Hence this implies that the token used by $\tr t_1$ is produced by $\tr{t_2}$. Furthermore, if we execute $\tr t_1$ we have that the token is in the place $\postS{\tr{t_1}}$ and this means that $\rev{\tr{t_2}}$ cannot be fired. Hence this case cannot happen.
}

\item $\rev{\tr{t_2}} \prec{ \tr{t_1}} $, this implies 
that $\postS{\rev{\tr{t_2}}}\cap \preS{\tr{t_1}} \neq \emptyset$,
and that $\preS{\tr{t_2}}\cap \preS{\tr{t_1}}\neq \emptyset$. The last says that $\tr{t_1}$ and $\tr{t_2}$ 
are in an immediate conflict.
Since we have $\tr{t_1};\rev{\tr{t_2}}$ in $\omega$ it means that in order to undo $\tr{t_2}$ the transition 
must have occurred before $\tr{t_1}$ in $\omega$. It is not possible that some other transition $\tr{t_3}$ 
produced a token to a place $\p a$ that was used by $\rev{\tr{t_2}}$: if it could happen it would mean that 
$\{\tr{t_2}, \tr{t_3}\}=\preS{\p a}$, so there is a backward conflict: contradiction.
Hence, $\tr{t_1}$ and $\tr{t_2}$ occurred before $\rev{\tr{t_2}}$ in $\omega$. Since $\tr{t_1}$ and $\tr{t_2}$
are in an immediate conflict, if one transition takes place the other cannot happen (as they share tokens 
in their preplaces). This contradicts that both $\tr{t_1}$ and $\tr{t_2}$ appear in $\omega$ before $\rev{\tr{t_2}}$.

	
\Comment{
\item $\tr{t_1}\#_0 \rev{\tr{t_2}} $ and by definition of $\#_0$ we have that 
$\preS{\tr{t_1}} \cap \preS{\rev{\tr{t_2}}}$ which implies $\preS{\tr{t_1}}\cap \postS{\tr{t_2}}$. For simplicity
we will consider transitions that consume one token, but the general case is similar.
Hence this implies that the token used by $\tr t_1$ is also used by $\tr{t_2}$. Furthermore, 
if we execute $\tr t_1$ we have that the token is in the place $\postS{\tr{t_1}}$ and this means 
that $\rev{\tr{t_2}}$ cannot be fired. Hence this case cannot happen.
}
\item $\tr{t_1}\#_0 \rev{\tr{t_2}} $ and by definition of $\#_0$ we have 
$\preS{\tr{t_1}} \cap \preS{\rev{\tr{t_2}}}$. Since $\tr{t_1};\rev{\tr{t_2}}$ appears in $\omega$, 
the firing $\tr{t_1}$ uses some tokens needed by $\rev{\tr{t_2}}$ to fire. Since there is no computation 
between $\tr{t_1}$ and $\rev{\tr{t_2}}$ in $\omega$ (that can replace the tokens needed by $\rev{\tr{t_2}}$),
$\rev{\tr{t_2}}$ cannot fire: contradiction. 

%	
\Comment{\item $\tr{t_1}\# \rev{\tr{t_2}} $ implies that
there exist $x$ and $y$ such that $x \prec \tr{t_1}$
and $y \prec \rev{\tr{t_2}}$ with $x \#_0 y$. But this is not possible, as $x$ and $y$ should be 
present in $\rev{\trace_1}$ which means they both
have executed before $\tr{t_1};\rev{\tr{t_2}}$.}

\item $\tr{t_1}\# \rev{\tr{t_2}}$, this implies that
there exist earlier $x$ and $y$ in $\omega$ such that $x \prec \tr{t_1}$
and $y \prec \rev{\tr{t_2}}$ with $x \#_0 y$. So we have $x$ and $y$ in an immediate conflict appearing in $\omega$
prior to subtrace $\tr{t_1};\rev{\tr{t_2}}$. We then show a contradiction as in case 2 above. 

\end{enumerate}

%If $\tr{t_1}\# \tr{t_2}$ we have two cases:
%either $\tr{t_1} = \tr{t_2}$ or not.
%%$\postS{\tr{t_1}}\cap \preS{\rev{\tr{t_2}}} \neq \emptyset$ we have two cases: either they are the same firing, that is $\tr{t_1} = \tr{t_2}$,
%%or not. 
%In the first case, by using the Loop Lemma (Lemma~\ref{lm:loop}) we can remove $\tr{t_1};\rev{\tr{t_1}}$ from $\trace$ obtaining a shorter trace. Then the results follows by applying the induction on a shorter trace.
%In the other case, 
%we have that either  
%$ (i)\ \postS{\tr{t_1}}\cap \preS{\rev{\tr{t_2}}} \neq \emptyset$
% or
% $ (ii)\ \preS{\tr{t_1}}\cap \postS{\rev{\tr{t_2}}} \neq \emptyset$
%.
%Since $\rev{\tr{t_2}}$
%is by construction the reverse firing of $\tr{t_2}$ (see Definition~\ref{lbl:rev_occ}),  
%$\postS {\tr t_1} \cap \preS{\rev{\tr t_2}} \neq \emptyset$ implies 
% $\postS {\tr {t_1}} \cap \postS{\tr {t_2}}\neq \emptyset $. 
% This means that there is a backward conflict between $\tr{t_1}$ and $\tr{t_2}$. By definition
% an occurrence net if free from backward conflicts. Moreover, by construction (see Definition~\ref{lbl:rev_occ}) the forward firing
% of the reversible net are the same of the original occurrence net, hence also in the reversible net there is no backward conflict among forward firings. Hence this case cannot happen.
 %
%
% In the case $(ii)$ we have that $\preS {\tr {t_1}} \cap \postS{\rev{\tr {t_2}}}\neq \emptyset $ implies
% $\preS {\tr {t_1}} \cap \preS{\tr {t_2}}\neq \emptyset $.
% For simplicity
%	we will consider transitions that consume one token, but the general case is similar.
% Hence this implies that the token used by $\tr t_1$ is produced by $\tr{t_2}$. Furthermore, if we execute $\tr t_1$ we have that the token is in the place $\postS{\tr{t_1}}$ and this means that $\rev{\tr{t_2}}$ cannot be fired. Hence this case cannot happen.
\end{proof}
 
\begin{lm}{\ref{lm:short}}
Let $\trace_1\ceq \trace_2$  with $\trace_2$ forward.
Then,  $\len{\trace_2} \leq \len{\trace_1}$.
\end{lm}
\begin{proof}
We prove this lemma by induction on the length of $\trace_1$. If $\trace_1$ is a forward trace we are already done. Otherwise by applying Lemma~\ref{lm:rearranging} we have that  $\trace_1 \ceq \rev\trace;\trace'$ (with both $\trace$, $\trace'$ \textit{forward}).
Consider the sub-trace $\rev{\tr{t_1}};\tr{t_2}$ with two successive firings with opposite directions
in $\rev\trace;\trace'$. Clearly
it is the only sub-trace of this form in 
$\rev\trace;\trace'$. 
%Let $\rev{\tr{t_1}};\tr{t_2}$ the only two successive transitions in $\trace_1$ with opposite direction.
Suppose $\preS{\rev{\tr{t_1}}} = m'$ and 
	$\postS{\rev{\tr{t_1}}} = m''$.
	 Since
$\trace_2$ is a forward only trace, this means that the marking $m'$ removed by $\rev{\tr{t_1}}$ 
have to be put back in $\trace_1$, otherwise this change would be visible in $\trace_2$ 
(since it is a forward only trace). Let $\tr{t_3}$ the earliest transition able to consume $m''$ 
and put back $m'$. This implies that $\tr{t_3} = \tr{t_1}$ since in occurrence nets there are no loops. 
Let us note that we can apply this reasoning to occurrence nets since we just consider forward firings. 
Moreover, all the transitions between $\rev{\tr{t_1}}$ and $\tr{t_3}$ can be swapped with $\tr{t_3}$, 
since they are concurrent with respect to $\tr{t_3}$. This is because all of them are forward transitions, 
occurrence nets are free from loops, and since $\tr{t_3}$ is the first firing after $\rev{\tr{t_1}}$ 
able to consume $m''$ and produce $m'$.
%
We can then apply the property of \m\ traces, and obtain an equivalent trace
where  $\rev{\tr{t_1}}$ and $\tr{t_3}$ are adjacent. Next, by applying $\ceq$, we can cancel them out 
(since $\tr{t_3} = \tr{t_1}$). Finally we conclude by applying the inductive hypothesis on a shorter trace.\qed
\end{proof}

\begin{tm}{\ref{th:causal}}
$$\trace_1 \ceq \trace_2 \text{ if and only if } (\rev{O},m_0)\red[\trace_1](\rev {O},m_n) \iff (\rev{O},m_0)\red[\trace_2](\rev{O},m_n)$$
\end{tm}

\begin{proof}
\noindent \textbf{$\Rightarrow$ direction}. If $\trace_1 \ceq \trace_2$  then $(N,m_0)\red[\trace_1](\rev{O},m_n) \iff (\rev{O},m_0)\red[\trace_2](\rev{O},m_n)$. 
First, notice that if $\trace_1\ceq \trace_2$ then it must be the case that $\trace_1$ can be transformed into $\trace_2$ (and vice versa) through $n \geq 0$ applications of the rules of $\ceq$. 
We then proceed by induction on $n$. In the base case, $n = 0$, we have that $\trace_1 \ceq \trace_2$ by applying $0$ times the rules of $\ceq$. Since $\ceq$ is an equivalence, this means that $\trace_1 = \trace_2$ which in turn implies that the traces are coinitial and cofinal. 
%
In the inductive case, we have that there exist $n$ traces $\trace^k$ (with $0 \leq k \leq n$) obtained as a result of applying the rules of $\ceq$ to $\trace_1$ exactly $k$ times; 
hence, $\trace^0 = \trace_1$ and $\trace^n = \trace_2$. 
We then have that $\trace^{n-1} \ceq \trace_2$, i.e., traces $\trace^{n-1}$ and $\trace_2$ differ in one axiom application; this means that we can decompose both traces as follows:
\begin{align*}
\trace^{n-1}= \trace_a;\trace';\trace_b && \trace_2= \trace_a;\trace'';\trace_b &&
\end{align*}
with $\trace'$ and $\trace''$ differing by just one application of $\ceq$. We have then three cases:
\begin{enumerate}
	\item $\trace' = \tr{t_1};\tr{t_2}$ and $\trace'' = \tr{t_2};\tr{t_1}$ with $\tr{t_1}\ co \ \tr{t_2}$
	\item $\trace' = \tr{t} ; \rev{\tr{t}}$ and $\trace'' =\voidt_m$ with $m$ the marking before firing $\tr{t}$
	\item $\trace' = \rev{\tr{t}} ; \tr{t}$ and $\trace'' = \voidt_m$  with $m$ the marking after firing $\tr{t}$
\end{enumerate}
In all cases it is easy to see that $\trace^{n-1}$ and $\trace_2$ are both coinitial and cofinal. By inductive hypothesis, $\trace_1 \ceq \trace^{n-1}$ implies that $\trace_1$ and $\trace^{n-1}$ are coinitial and cofinal; since $\trace^{n-1} \ceq \trace_2$ implies that they are coinitial and cofinal, we can conclude that also $\trace_1$ and $\trace_2$ are coinitial and cofinal if $\trace_1 \ceq \trace_2$.
\\[.4cm]
\noindent \textbf{$\Leftarrow$ direction}. We have to show that
if $(\rev{O},m_0)\red[\trace_1](\rev{O},m_n)$ and $(\rev{O},m_0)\red[\trace_1](\rev{O},m_n)$ then $\trace_1 \ceq \trace_2$.
By Lemma~\ref{lm:rearranging} we know that the two traces can be written as composition of a backward trace and a forward one. The proof is by lexicographic induction on the sum of the lengths of $\trace_1$ and 
$\trace_2$ and on the distance between the end of $\trace_1$ and the earliest pair of transitions $\tr{t_1}$ in $\trace_1$ and $\tr{t_2}$ in $\trace_2$ which are not equal. If all the transitions are equal then we are done. Otherwise we have to consider four cases depending on the direction of the two transitions.
%The proof is by induction on $\trace_1$ and the 
%$len(\trace_1)+len(\trace_2)$, and on the distance between the end of $\trace_1$ and the earliest pair of differing reductions $(O,m')\red[\tr{t_1}] (O,m_1)$ and $(O,m'')\red[\tr{t_2}] (O,m_2)$ with
%$\tr{t_1}\in \trace_1$ and $\tr{t_2}\in \trace_2$. If there is no such a pair, then $\trace_1$ and $\trace_2$ are equal and the theorem trivially holds. Otherwise we have to consider four cases depending on the directions of $\tr{t_1}$
%and $\tr{t_2}$. We use the Lemma~\ref{lm:rearranging}, which ensures that any trace can be written as a composition of a backward sub-trace followed by a forward sub-trace.
\begin{description}
	\item[$\tr{t_1}$ forward and $\tr{t_2}$ backward]: we have that
	$\trace_1 = \rev\trace;\tr{t_1};\trace'$ and $\trace_2 = \rev\trace;\tr{t_2};\trace''$
	with $\rev\trace$  the common backward subtrace and $\tr{t_1};\trace'$ 
	a forward trace. By hypothesis we have that $\trace_1$ and $\trace_2$ are coinitial and cofinal and
	this implies that also $\tr{t_1};\trace'$ and $\tr{t_2};\trace''$ are coinitial and cofinal.
	By applying Lemma~\ref{lm:short}  on the trace $\tr{t_2};\trace''$ we obtain a shorter equivalent 
	forward trace and therefore $\trace_2$ has a shorter causally equivalent forward trace. We can then conclude by induction (on a shorter trace).
	\item[$\tr{t_1}$ backward and $\tr{t_2}$ forward]: similar to the previous case.
	\item[$\tr{t_1}$ forward and $\tr{t_2}$ forward] By assumption the two transitions are different, that  $\tr{t_1} \neq \tr{t_2}$. We can decompose the two traces as follows $\trace_1 = \trace;\tr{t_1};\trace^1$
	and $\trace_2 = \trace;\tr{t_2};\trace^2$. Moreover all the firings in $\trace^i$ are forward.
	If $\tr{t_1}$ and $\tr{t_2}$ are in conflict, this means that $\preS{\tr{t_1}} \cap \preS{\tr{t_2}} \neq \emptyset$. Since the two traces are cofinal, this means that the effect
	of $\tr{t_1}$ will remain visible till the end, so we have:
\begin{align*}
&	(\rev{O},m_0) \red[\trace] (\rev{O},m) \fred[\tr{t_1}] (\rev{O},m_1) \fred[\trace^1] (\rev{O},m_f) \\
&	(\rev{O},m_0) \red[\trace] (\rev{O},m) \fred[\tr{t_2}] (\rev{O},m_2) \fred[\trace^2] (\rev{O},m_f) 
\end{align*}		
	with $m_1 \neq m_2$. But this implies that in $\trace^2$ there will be a firing
	able to put produce the tokens necessary to $\tr{t_1}$ to fire, which implies
	the existence of a loop. Since we are just considering the forward firing of a reversible occurrence net,
	they are by construction the transition of an occurrence net, which by definition is acyclic. So this case cannot happen. Hence we have that $\tr{t_1}\ co \ \tr{t_2}$, and that $\tr{t_1}\in \trace^2$.
We now have to show that $\tr{t_1}$ is concurrent with all the firings
	between $\tr{t_2}$ and itself. We can apply the same reasoning as before (absence of cycles)
	and by applying several times the property of \m\ traces we can rearrange $\trace_2$ in such
	a way that $\trace_2 =  \trace;\tr{t_1};\tr{t_2};\trace^3$, where $\trace^3$ is $\trace^2$ without $\tr{t_2}$.
	We then have $\trace_1 = \trace;\tr{t_1};\trace^1$ and 
	$\trace_2 = \trace;\tr{t_1};\tr{t_2};\trace^3$. They have the same length as before, but the first pair of
	discording firings is closer to the end of the trace. The thesis follows by inductive hypothesis.
	\item[$\tr{t_1}$ backward and $\tr{t_2}$ backward]  the two firings cannot remove the same token,
	since this would mean that by considering their forward variants there is a backward conflict, which by
	definition occurrence net is impossible. Since the two traces are coinitial and cofinal, then either
	there exists in $\trace_1$ a firing which is the forward version of $\tr{t_1}$ or there exists in $\trace_2$
	the firing $\tr{t_1}$. In the first case, $\tr{t_1}$ is concurrent with all the backward transitions following it (in the trace) but with the ones which do the same firing. All these transitions have a corresponding forward move in the trace, otherwise we would have that the effect of $\tr{t_1}$ is visible till the end, contradicting the 
	hypothesis that $\trace_1$ and $\trace_2$ are coinitial and cofinal. We then select the last of such
	firing and swap it with all the backward firings following it, in order to make it the very last backward firing of the trace. We then select the first forward firing which is its opposite, and since it is concurrent with all the forward firings proceeding it, we can swap them in such a way to have it as the very first forward firing.
	We can then apply the axiom  $\rev{\tr{t_1}};\tr{t_1} \ceq \voidt_m$ with $m$ being the marking of the net before firing $\rev{\tr{t_1}}$. We then obtain a shorter trace, equivalent to $\trace_1$. The thesis then follows by induction.	
	
	In the second case, the reasoning is similar to the case in which both $\tr{t_1}$
	and $\tr{t_2}$ are forward.
\end{description}
\end{proof}

\begin{tm}[\ref{th:rev_sem}]
	Let $O$ be an occurrence net and $m_0$ an initial marking. Then,
	
	\begin{align*}
		(\rev O,m_0) \red[]^* (\rev O, m') \iff (\rev O,m_0) \fred[]^*
		(\rev O, m')
	\end{align*}
\end{tm}
\begin{proof}
	The $\Leftarrow$ case trivially holds, as $\fred[] \subset \red[]$.
	In the other case we have that
	  $(\rev O,m_0) \red[\trace] (\rev O, m')$. By using Lemma~\ref{lm:rearranging} we have that
	  	  $\trace \ceq \rev{\trace_1};\trace_2$ with $\trace_2$ forward. Since $\trace \ceq \rev{\trace_1};\trace_2$, by Theorem~\ref{th:causal}
	  we have that also $(\rev O,m_0) \bred[\trace_1] \fred[\trace_2] (\rev O, m')$. Let us note that $m_0$ is an initial marking, and this implies that no backward computations can take place from $(\rev O, m_0$) meaning that $\trace_1 = \voidt_{m_0}$. Hence we have that
	  $\trace \ceq \trace_2$ with $\trace_2$ a forward trance.
	  By Theorem~\ref{th:causal} we have that
	  $(O,m_0)\red[\trace] (O,m')$ implies 
	  $(O,m_0) \fred[\trace_2] (O,m')$ as desired.
\end{proof}



